Learning Temporal Dependence from Time-Series Data with Latent Variables

We consider the setting where a collection of time series, modeled as random processes, evolve in a causal manner, and one is interested in learning the graph governing the relationships of these processes. A special case of wide interest and applicability is the setting where the noise is Gaussian and relationships are Markov and linear. We study this setting with two additional features: firstly, each random process has a hidden (latent) state, which we use to model the internal memory possessed by the variables (similar to hidden Markov models). Secondly, each variable can depend on its latent memory state through a random lag (rather than a fixed lag), thus modeling memory recall with differing lags at distinct times. Under this setting, we develop an estimator and prove that under a genericity assumption, the parameters of the model can be learned consistently. We also propose a practical adaption of this estimator, which demonstrates significant performance gains in both synthetic and real-world datasets.

==> Sections/Other/Analysis.tex <==
\section{Analysis}\label{sect:analysis}

%We intend to learn matrices $A$, $B$ and $D$ from the observations. Matrix $A$ is of particular interest, since it captures the underlying causal graph of the process. For this, we try to derive equations in terms of sample covariances of the observations and system parameters. 
For learning the system parameters, we derive equations in terms of sample covariances of the observations and system parameters. 

\textcolor{red}{Assume $x_0$ and $z_0$ are zero vectors. Thus, according to Equ.~\ref{Eq:Mod}, $x_t$ and $z_t$ are multivariate normal distributed with zero mean.} 
Let $\Sigma_{ZX_i}=\Sigma_{Z_t,X_{t-i}} = \mathbb{E}[z_tx^T_{t-i}]$ denote the cross-covariances of $x_t$ and $z_t$. Note that due to stationarity, we have $\Sigma_{ZX_i}=\Sigma_{Z_{t-j},X_{t-i-j}}$ for any integer $j$.
For simplicity, we write $\Sigma_{X}=\Sigma_{X_0}$ and $\Sigma_{ZX}=\Sigma_{{ZX}_0}$. 
Let $\tau_1$ and $\tau_2$ be vectors. We define the $(i,j)$-th element of $\Sigma_{Z_{\tau_1}X_{\tau_2}}$ as 
$\Sigma_{Z_{\tau_1}X_{\tau_2}}(i,j) = \mathbb{E}[z_{t-\tau_1(i)}(i)x^T_{t-\tau_2(j)}(j)]=\mathbb{E}[z_{t}(i)x^T_{t-\tau_2(j)+\tau_1(i)}(j)]$. 
We also denote the covariances of the state and observation noises by $\Sigma_V$ and $\Sigma_W$, respectively.

Since $\Theta_t$ is i.i.d., for simplicity we drop the subscript of $\Theta_t$, when it does not lead to confusion.
Let us denote $\Sigma_{UY_{\Theta}}=\mathbb{E}_{t,\Theta}[u_ty_{t-\Theta}^T]$, where $u$ and $y$ are time series vectors and $\Theta$ is as defined in Equ.~\ref{Eq:Sys}. Note that $\Sigma_{UY_{\Theta}}$ is not random. 
We use the following two Lemmas for deriving the equations and in proofs.
\begin{lem}
	$\Sigma_{UY_{\Theta}}=\sum_{\theta=0}^{\theta_{\max}} {q_{\theta}\Sigma_{UY_{\theta}}}.$
\end{lem}
\begin{proof}
	We have
	\begin{align}
	\nonumber \Sigma_{UY_{\Theta}}(i,j)&=\mathbb{E}_{t,\Theta}[u_t(i)y_{t-\Theta(j)}^T(j)]\\
	\nonumber &=\mathbb{E}_{\Theta}[\mathbb{E}_t[u_t(i)y^{T}_{t-\Theta(j)}(j) | \Theta(j)=\theta]]\\
	\nonumber &=\mathbb{E}_{\Theta}[\Sigma_{UY_{\theta}}(i,j)]\\
	\nonumber &=\sum_{\theta=0}^{\theta_{\max}} {q_{\theta}\Sigma_{UY_{\theta}}(i,j)}.
	\end{align}
	
\end{proof}

Let $y_t = u_{t-\Theta}$ and $u_{t} = Gu_{t-1}$, where $G$ is a $p\times p$ matrix. Note that $y_t \neq Gu_{t-\Theta-1}$, since each coordinate of $u$ is shifted randomly independently, and, thus, the matrix $G$ applies to elements of $u$ in different times. The following Lemma shows that we still have $\mathbb{E}_t[y_{t}y_{t-k}^T]=\mathbb{E}_{t,\Theta}[Gu_{t-\Theta-1}y_{t-k}^T]=\mathbb{E}_{t,\Theta}[Gu_{t}y_{t-k+\Theta+1}^T]$.
 
\begin{lem}\label{lem:G}
	Let $y_t$, $u_t$ and $G$ be defined as above. We have 	$\mathbb{E}_t[y_{t}y_{t-k}^T]=G\Sigma_{UY_{k-\Theta-1}}$.
\end{lem}
\begin{proof}
	Let us denote $\Sigma=\mathbb{E}_t[y_{t}y_{t-k}^T]$. We have
	\begin{align}
	\nonumber \Sigma(i,:)&=\mathbb{E}_{t,\Theta}[u_{t-\Theta(i)}(i)y_{t-k}^T]\\ 
	\nonumber &=\mathbb{E}_{t,\Theta}[G(i,:)u_{t-\Theta(i)-1}y_{t-k}^T]\\
	\nonumber&=\mathbb{E}_{\Theta}[\mathbb{E}_t[G(i,:)u_{t-\Theta(i)-1} y_{t-k}^{T}| \Theta(i)=\theta]]\\
	\nonumber&=\mathbb{E}_{\Theta}[G(i,:)\Sigma_{UY_{k-\theta-1}}]
	\end{align}
	where $\Sigma(i,:)$ and $G(i,:)$ denote the $i$-th row of $\Sigma$ and $G$, respectively. Therefore, we have $\Sigma=\mathbb{E}_{\Theta}[G\Sigma_{UY_{k-\theta-1}}]=G\Sigma_{UY_{k-\Theta-1}}$.
\end{proof}

%\begin{lem}
%	For any fixed $\Theta \geq 0$, we have:
%	\begin{align}
%	\Sigma_{X_{1}} &= (A+D)\Sigma_{X}-AD\Sigma_{X_{1}}^T+B\Sigma_{X_{\Theta}}^T -A\Sigma_W \label{Eq:1}\\
%	\Sigma_{X_{i+1}} &= (A+D)\Sigma_{X_i}-AD\Sigma_{X_{i-1}}+B\Sigma_{X_{i-\Theta}}, i\geq 1.\label{Eq:i} \\
%	\nonumber \textcolor{red}{\Sigma_{X_{i+1}}} &= (A+D)\Sigma_{X_i}-AD\Sigma_{X_{i-1}}+B\Sigma_{X_{i-\Theta}}\\
%		&-\mathbf{1}_{i=0}A\Sigma_W, i\geq 0.
%	\end{align}
%\end{lem}
%\begin{proof}
%\end{proof}

%For random $\Theta$, we have to replace $\Sigma_{i-\Theta}$ with $\mathbb{E}_{\Theta}(\Sigma_{i-\Theta})$. 
%Similarly, for the case that $\Theta$ is random, we have the following Lemma.
\begin{lem}
	\begin{align}\label{Eq:opt1}
	\Sigma_{X_{i+1}}= (A+D)\Sigma_{X_i} -AD&\Sigma_{X_{i-1}}+B \Sigma_{X_{i-\Theta}} \;\; , i\geq \max(\theta_{\max},1).
	\end{align}
\end{lem}
\begin{proof}
	We have
	\begin{align}
	&\Sigma_{X_{i}}= \Sigma_{ZX_{i-\Theta_t}} + D\Sigma_{X_{i-1}}, i\geq 1,\label{Eq:eq_xi}\\
	&\Sigma_{X_{i+1}}= A\Sigma_{ZX_{i-\Theta_t}} + B\Sigma_{X_{i-\Theta_t}} + \Sigma_{V_{\Theta_t}X_{i+1}} + D\Sigma_{X_{i}}, i\geq 0,\label{Eq:eq_xi+1}
	\end{align}
	We obtain Equ.~\ref{Eq:eq_xi} by multiplying $x_{t-i}^T$ to the second equation of the model \ref{Eq:Mod} and taking the expectation. Since $w_t$ is independent of $x_{t-i}, i \geq 1$, we have $\Sigma_{W_tX_{t-i}}=0$. 
	We also obtain Equ.~\ref{Eq:eq_xi+1} by first multiplying $x_{t-i-1}^T$ to the second equation of the model and taking the expectation, and then replacing $\Sigma_{ZX_{i+1-\Theta_t}}$ from the first equation, using Lemma~\ref{lem:G}.
	
	To derive equations which are independent of the structure of $\Sigma_V$, we need to find $i$ such that $\Sigma_{V_{\Theta_t}X_{i+1}}$ is zero. We have
	\begin{align}
	&\Sigma_{V_{\Theta_t}X_{i+1}}=\Sigma_{V_{\Theta_t}Z_{i+2+\Theta_{t-(i+1)}}}A^T+\Sigma_{V_{\Theta_t}X_{i+2+\Theta_{t-(i+1)}}}B^T+\Sigma_{V_{\Theta_t}V_{i+1+\Theta_{t-(i+1)}}}.
	\end{align}	
	Recall that $v_t$ is independent of $z_{t-i}$ and $x_{t-i}$ for $i > 0$. Thus, for the first and second terms to be zero, we must have $\Theta_t<i+2+\Theta_{t-(i+1)}$. Since $\Theta$ lies in $[0\,,\,\theta_{\max}]$ and is i.i.d., we must have $i>\theta_{\max}-2$.
	For the third term to be zero, we must have $\Theta_t \neq i+1+\Theta_{t-(i+1)}$ and, since $\Theta_t-\Theta_{t-(i+1)} \in [-\theta_{\max}\,,\,\theta_{\max}]$, we must have $i > \theta_{\max}-1$. 
	%
	Therefore, for $i\geq \theta_{\max}$, $\Sigma_{V_{\Theta_t}X_{i+1}}=0$. By replacing $\Sigma_{ZX_{i-\Theta_t}}$ in Equ.~\ref{Eq:eq_xi+1} from Equ.~\ref{Eq:eq_xi}, we obtain Equ.~\ref{Eq:opt1}.
\end{proof}

Let $K_1 = B^{-1}(A+D)$ and $K_2=B^{-1}AD$. 
We can write \ref{Eq:opt1} as follows
\begin{align}\label{Eq:opt2}
B^{-1}\Sigma_{X_{i+1}}- K_1\Sigma_{X_i} +K_2\Sigma_{X_{i-1}} - \Sigma_{X_{i-\Theta}}=0 \;\; , i\geq \max(\theta_{\max},1).
\end{align}

Now, we are ready to prove Claim~\ref{clm:alg}.

First note that, for $\max(\theta_{\max},1) \leq i \leq (2\theta_{\max}+1)$, Equ.~\ref{Eq:opt2} forms a linear system of equations. When $T\rightarrow \infty$, we have the exact estimation of covariances. Therefore, 



Clearly $S \in \underset{B',K_1,K_2,q}{\text{arg\,min}}$, but show that $S = \underset{B',K_1,K_2,q}{\text{arg\,min}}$. If we have two solutions, any convex combinations is also a solution. 

Why sign-saprsity pattern of $K_1$ not $K_2$?

Why this convex (relaxed)?

Note that, for learning the parameters, we are not using the matrix inversion that is used in the proof~\ref{apx:ProofThm1}; therefore, the above formulation does not require the assumptions that $\theta_{\max} > 0$ or that all $q_i, i\in [0\,,\,\theta_{\max}],$ must be non-zero. 

==> Sections/Other/DELETED.tex <==
We consider a linear dynamical system model in which we use the observations from the previous time step as inputs for the current time step. The model is as follows:
\begin{align}\label{Eq:Sys}
\begin{cases}
z_t = Az_{t-1} + Bx_{t-1} + v_t \\
x_t = Cz_{t} + Dx_{t-1} + w_t
\end{cases}
\end{align}
where $z$ denotes the hidden state variables and $x$ is the observations. This model is introduced in \cite{rangel2005modeling,beal2005bayesian} for gene expression, as a state-space model with inputs (which are the past observations), where the dimensions of the hidden variables is much smaller then the dimension of the observations, i.e., $|z|\ll|x|$. 

In this paper, we consider the setting where each observed variable has a corresponding hidden state, i.e., $|x|=|z|$. This hidden component helps to capture the effect of unseen factors on observations and, as a result, simplify the causal dependencies among the observations.
%captures the temporal behaviour of the variable and summarizes the information from the past. 
For this, we assume that each hidden component has a causal relationship with only itself and its corresponding observation (i.e. matrices $A$, $B$ and $C$ are diagonal), and each observation interacts with only a few other observations (i.e. matrix $D$ is sparse), and all matrices have positive diagonals. Also, the state and observation noise are independent and distributed as multivarite normal \textcolor{red}{iid?}. 

%We assume that each variable in $x_t$ depends on some few components of $x_{t-1}$ and also on its corresponding hidden component, and each variable in $z_t$ depends only on the past of itself and its corresponding observation, i.e., $A$, $B$ and $C$ are diagonal, and $D$ is sparse. 

The model can be written as:
\begin{align}\label{Eq:Mod1}
& \begin{bmatrix}
z_{t} \\
x_{t}
\end{bmatrix}=
H
\begin{bmatrix}
z_{t-1} \\
x_{t-1}
\end{bmatrix} 
+n_t
\end{align}
where $H=\begin{bmatrix}
A & B\\
CA & CB+D
\end{bmatrix}$ and 
$n_t =\begin{bmatrix}
v_{t} \\
w_t+Cv_{t}
\end{bmatrix}$
and therefore
$\Sigma_N =
\begin{bmatrix}
\Sigma_v & \Sigma_vC^T\\
C\Sigma_v & \Sigma_w+C\Sigma_vC^T
\end{bmatrix}$, where $\Sigma_V$ and $\Sigma_W$ denote the covariances of state and observation noise, respectively, and $\Sigma_N$ is the covariance of $n_t$.

We propose the following model:
\begin{align}\label{Eq:Sys}
\begin{cases}
z_t = Az_{t-1} + Bx_{t-1} + V_t \\
x_t = z_{t-\tau_t} + Dx_{t-1} + W_t
\end{cases}
\end{align}
where $\tau_t \in \{\mathbb{Z}\}^p$ is a random vector, with the constraint that for the $i$-th element we have $\tau_t^i \leq \tau_{t-1}^i+1$, meaning that once an observation depends on $z_{t_1}^i$, future observations can only depend on $z_{t_2}^i, t_2\geq t_1$.

\subsection{Structural Properties of the Model}

The three important properties in the state-space representation of time series are stability, controllability, and observability \cite{rangel2005modeling}. 
Let us define a new state vector to be $u_t = [z_t^T \; x_t^T]^T$. Then the model in Equ.~\ref{Eq:Mod1} can be written as:
\begin{align}\label{Eq:Mod1new}
u_{t+1}&=Hu_{t}+N_{t+1}\\
x_t &= F U_t
\end{align}
where $F=[0 \; I]$, and $0$ and $I$ are $p\times p$ zero and identity matrices, respectively.


\subsubsection{Stability}  It must be ensured that the model does not cause the system to diverge to infinity. In order to maintain stability, we require that the spectral radius of the dynamics be less than or equal to 1. That is, we must have $\max(\lambda(H))\leq 1$, where $\lambda$ denotes the vector of eigenvalues for the matrix $H$.

\subsubsection{Controllability} Controllability is the requirement that the state vector $z_t$ can be controlled from any arbitrary initial state to any other arbitrary final state in finite time.
This would need to be accomplished by selecting $v_t$ to evolve in time in a particular way. Since we assume that the noise covariance for $v_t$ is nonsingular, the system is controllable if and only if $[I,H,H^2,\ldots,H^{2p-1}]$ is full rank. 

\subsubsection{Observability} Observability is the dual of controllability and is considered in terms of the observed variables $x_t$. We say that the system is observable if given zero noise, we can reconstruct the initial state vector from a full sequence of $x_t$.
This is achieved if and only if $[F^T,H^TF^T,(H^2)^TF^T,\ldots,(H^{2p-1})^TF^T]$ has full rank.

\subsection{Identifiability}
Any coordinate transformation of hidden variables as $z'_t=Tz_t$, where $T$ is any nonsingular matrix, will generate observations that are identically distributed with those in Equ.~\ref{Eq:Mod1}. The new model can be represented as
$$H'=
\begin{bmatrix}
TAT^{-1} & TB\\
CAT^{-1} & CB+D
\end{bmatrix}.$$

To deal with the unknown coordinate transformation, we must fix one of the matrices related to the hidden components. If we set $C$ to be the identity matrix, then $T$ can only be identity. The modified model is:
\begin{align}\label{Eq:Mod}
\begin{cases}
z_t = Az_{t-1} + Bx_{t-1} + v_t \\
x_t = z_{t} + Dx_{t-1} + w_t
\end{cases}
\end{align}
and it can be written similar to Equ.~\ref{Eq:Mod1} with
$ H=\begin{bmatrix}
A & B\\
A & B+D
\end{bmatrix}
$ and $N_t =\begin{bmatrix}
v_{t} \\
w_t+v_{t}
\end{bmatrix}$
and therefore
$\Sigma_N =
\begin{bmatrix}
\Sigma_v & \Sigma_v\\
\Sigma_v & \Sigma_w+\Sigma_v^T
\end{bmatrix}.$\\

==> Sections/Other/EM.tex <==
\section{EM}

\subsection{Kalman}
Kalman in steady state:

\subsection{Estimation}


==> Sections/Other/Noise.tex <==
\subsection{Noise Covariance Estimation}
We have 
\begin{align}
%& \Sigma_{X_{t,t-1}} =\Sigma_{Z_tX_{t-1}} + D\Sigma_{X} \label{Eq:N1}\\
& \Sigma_{Z_tX_{t-1}} =A\Sigma_{ZX} + CB\Sigma_{X} \label{Eq:N2}
\end{align}
%
Also:
\begin{align}\label{Eq:N3}
\nonumber & E[X_tX_{t}^T] = E[Z_{t}X_{t}^T] + DE[X_{t-1}X_{t}^T] + E[W_tX_{t}^T] \\
\nonumber & \Rightarrow E[X_tX_{t}^T] = E[Z_{t}X_{t}^T] + DE[X_{t-1}X_{t}^T] + E[W_t(Z_{t}+DX_{t-1}+W_t)^T] \\
 & \Rightarrow \Sigma_{X} =\Sigma_{ZX} + D\Sigma_{X_{t-1}X_{t}} + \Sigma_W
\end{align}
%
And:
\begin{align}\label{Eq:N4}
& \Sigma_{X_{t-1}X_t} =\Sigma_{Z_{t-1}X_t} + D\Sigma_{X_{t-2}X_{t}} + \Sigma_W(CB+D)^T
\end{align}
%
And:
\begin{align}\label{Eq:N5}
\nonumber & E[Z_tX_{t}^T] = AE[Z_{t-1}X_{t}^T] + CBE[X_{t-1}X_{t}^T] + E[CV_tX_{t}^T] \\
\nonumber & \Rightarrow E[Z_tX_{t}^T] = AE[Z_{t-1}X_{t}^T] + CBE[X_{t-1}X_{t}^T] + E[CV_t\big(AZ_{t-1}+(CB+D)X_{t-1} +CV_t+ W_t\big)^T] \\
 & \Rightarrow \Sigma_{ZX} =A\Sigma_{Z_{t-1}X_t} + CB\Sigma_{X_{t-1}X_{t}} + C\Sigma_VC^T
\end{align}
%
Knowing matrices $A$, $CB$ and $D$, and using Equs. \ref{Eq:S1}, \ref{Eq:N2}, \ref{Eq:N3}, \ref{Eq:N4} and \ref{Eq:N5}, we can obtain $\Sigma_W$ and $\Sigma_V'$ as follows:
\begin{align}\label{Eq:N6}
& \Sigma_{W} =A^{-1}\big((CB+D+A)\Sigma_{X} -\Sigma_{X_{t}X_{t-1}}\big) -D\Sigma_{X_{t-1}X_t} \\
& \Sigma_{V'} = \Sigma_{X} - (CB+D+A)\Sigma_{X_{t-1,t}} + AD\Sigma_{X_{t-2}X_t} -\Sigma_W+A\Sigma_W(CB+D)^T
\end{align}\\*

%From Equs~\ref{Eq:N1}, \ref{Eq:N2} and \ref{Eq:N3}, we can write:
%\begin{align}\label{Eq:N4}
% & \Sigma_{X} =(CB+D+CAC^{-1})\Sigma_{X_{t-1,t}} - CAC^{-1}D\Sigma_{X_{t-2}X_t} + C\Sigma_VC^T+\Sigma_W-CAC^{-1}\Sigma_W(CB+D)^T
%\end{align}
%
%Assuming that $A$ and $C$ are diagonal and $V'=CV$, we have:
%\begin{align}\label{Eq:N5}
% & \Sigma_{X} =(CB+D+A)\Sigma_{X_{t-1,t}} - AD\Sigma_{X_{t-2}X_t} + \Sigma_{V'}+\Sigma_W-A\Sigma_W(CB+D)^T
%\end{align}
%
%If we can recover the matrices $A$, $CB$ and $D$ from Equ.~\ref{Eq:Opt1}, we can form the following optimization problem to find $\Sigma_{V'}$ and $\Sigma_W$:
%
%We solve the following optimization problem:
%\begin{align}\label{Eq:Opt2}
% (\Sigma_1^*,\Sigma_2^*)=&  argmin_{\Sigma_1, \Sigma_2} \|\Sigma_{X} -(CB+D+A)\Sigma_{X_{t-1,t}} + AD\Sigma_{X_{t-2}X_t} - \Sigma_1-\Sigma_2+A\Sigma_2(CB+D)^T  \\
%\nonumber & \mbox{s.t. } \Sigma_1 \mbox{ and } \Sigma_2 \mbox{ are positive semidefinite.}
%\end{align}
%Then we let $\Sigma_{V'}=\Sigma_1^*$ and $\Sigma_W = \Sigma_2^*$.


==> Sections/Other/Parameter2.tex <==
Throughout our analysis and proofs, we use the following equations derived from the system equations~\ref{Eq:Mod}.
\begin{align}
\nonumber \Sigma_Z &= A\Sigma_ZA^T+A\Sigma_{ZX}B^T+B\Sigma_{XZ}A^T+B\Sigma_XB^T \\
& \;\;\; +\Sigma_V \label{Eq:z}\\
\nonumber \Sigma_X &= A\Sigma_ZA^T+A\Sigma_{ZX}(B+D)^T+(B+D)\Sigma_{XZ}A^T \\
& \;\;\; +(B+D)\Sigma_X(B+D)^T+\Sigma_V+\Sigma_W \label{Eq:x}\\
\Sigma_{ZX}&=\Sigma_Z+A\Sigma_{ZX}D^T+B\Sigma_XD^T \label{Eq:zx} \\
\Sigma_{ZX_1}&=A\Sigma_{ZX}+B\Sigma_X. \label{Eq:zx1}
\end{align}

%Using Equ.~\ref{Eq:Mod}, we have:
%\begin{align}
%x_t = & Dx_{t-1} +z_t+ w_t \label{Eq:S11}\\
%= & Dx_{t-1} + Bx_{t-1} +Az_{t-1}+ w_t+v_t \\
%= & Dx_{t-1} + Bx_{t-1} +ABx_{t-2} +A^2 z_{t-2} \\
%\nonumber  & \;\;\;+ w_t+v_t+Av_{t-1} \\
%\nonumber & \vdots \\
%\nonumber= & Dx_{t-1} + \Sigma_{i=1}^{\tau} {A^{i-1}Bx_{t-i}} +A^\tau z_{t-\tau} \\
%& \;\;\;+ w_t+\Sigma_{i=1}^{\tau} {A^{i-1}v_{t-i+1}},\tau \geq 1.\label{Eq:S1}
%\end{align}
%Note that the noise term in Equ.~\ref{Eq:S1} is independent of $x_{t-\tau}$ and $z_{t-\tau}$. 

Let us denote $K_1=A+B+D$ and $K_2=AD$. Note that the terms $K_1$ and $K_2$ are sparse, with the same sparsity pattern. We have the following Lemma. 

\begin{lem}
	We have
	\begin{align}
	\Sigma_{X_{1}}&= K_1\Sigma_{X} -K_2\Sigma_{X_{1}}^T-A\Sigma_W \label{Eq:S6}
	\end{align}	
\end{lem}
\begin{proof}
	Using Equ.~\ref{Eq:Mod}, we have: 
	\begin{align}
	\nonumber x_t = & Dx_{t-1} + \sum_{i=1}^{\tau} {A^{i-1}Bx_{t-i}} +A^\tau z_{t-\tau} \\
	& \;\;\;+ w_t+\sum_{i=1}^{\tau} {A^{i-1}v_{t-i+1}},\tau \geq 0.\label{Eq:S1}
	\end{align}
	Note that in Equ.~\ref{Eq:S1} the noise term is independent of $x_{t-\tau}$ and $z_{t-\tau}$, for $\tau \geq 1$. Multiplying Equ.~\ref{Eq:S1} by $x_{t-\tau}, \tau \geq 1,$ and averaging over time, we obtain:
	\begin{align}\label{Eq:S2}
	\Sigma_{X_{\tau}}= D\Sigma_{X_{\tau-1}} + \sum_{i=1}^{\tau} {A^{i-1}B \Sigma_{X_{\tau-i}}} +A^\tau \Sigma_{ZX},\tau \geq 1.
	\end{align}
	Also, multiplying Equ.~\ref{Eq:S1} for $\tau=0$ by $x_t$ and averaging over time, we get:
	\begin{align}\label{Eq:S4}
	\Sigma_{X}= D\Sigma_{X_{1}}^T+\Sigma_{ZX}+\Sigma_W.
	\end{align}
	Using Equ.~\ref{Eq:S2} for $\tau=1$ and Equ.~\ref{Eq:S4}, we get the result.
\end{proof}

\begin{lem}
	We have
	\begin{align}
	\Sigma_{X_{i}}&= K_1\Sigma_{X_{i-1}} -K_2\Sigma_{X_{i-2}}, i\geq 2. \label{Eq:S3}
	\end{align}	
\end{lem}
\begin{proof}
	Using Equ.~\ref{Eq:S2}, we can write: (Proof by induction)
\end{proof}

Using Equ.~\ref{Eq:S3} for $i=2$ and $3$, we get:
\begin{align}\label{Eq:Mat23}
\begin{bmatrix}
\Sigma_{X_2} & \Sigma_{X_3}
\end{bmatrix}=
\begin{bmatrix}
K_1 & -K_2
\end{bmatrix}M_{2,3}.
\end{align}
where
\begin{align}
M_{2,3}=
\begin{bmatrix}
\Sigma_{X_1} & \Sigma_{X_{2}}\\
\Sigma_{X}  & \Sigma_{X_1} 
\end{bmatrix}.
\end{align}

\begin{lem}\label{lm:instance}
	There exists an instance for which $M_{23}$ is full-rank. 
\end{lem}
\begin{proof}
	Let $A=\frac{1}{2}I$, $B=\frac{1}{4}I$, and $D=\frac{1}{4}I$. Then, we have:
	\begin{align}
	\Sigma_X&=\frac{576}{119}\Sigma_V+\frac{208}{119}\Sigma_W \\
	\Sigma_{X_1}&=\frac{512}{119}\Sigma_V+\frac{132}{119}\Sigma_W \\
	\Sigma_{X_2}&=\frac{440}{119}\Sigma_V+\frac{106}{119}\Sigma_W.
	\end{align}
	If we let $\Sigma_V=\Sigma_W=I$, then $\Sigma_X=\frac{784}{119}I$, $\Sigma_{X_1}=\frac{644}{119}I$, and $\Sigma_{X_2}=\frac{546}{119}I$, implying that there exists an instance for which both matrices $M_{12}$ and $M_{23}$ are full-rank. 
\end{proof}

\begin{thm}\label{Th:M23}
	the matrix $M_{23}$ is full-rank with probability one. 
\end{thm}
\begin{proof}
	Using Equations~\ref{Eq:z},~\ref{Eq:x} and \ref{Eq:zx} and applying the equality~\ref{Eq:kron}, we can write:
	\begin{align}
	&\nonumber (I-A\otimes A)\mathsf{V}_Z = (B\otimes A)\mathsf{V}_{ZX} +(A\otimes B)\mathsf{V}_{XZ} \\
	&+(B\otimes B)\mathsf{V}_{X}+\mathsf{V}_V\\
	&\nonumber (I-(B+D)\otimes (B+D))\mathsf{V}_X = (A\otimes A)\mathsf{V}_{Z}\\
	& +((B+D)\otimes A)\mathsf{V}_{ZX}+(A\otimes (B+D))\mathsf{V}_{XZ}+\mathsf{V}_V+\mathsf{V}_W \\
	& (I-D\otimes A)\mathsf{V}_{ZX} = \mathsf{V}_{Z} +(D\otimes B)\mathsf{V}_{X} \\
	& (I-A\otimes D)\mathsf{V}_{XZ} = \mathsf{V}_{Z} +(B\otimes D)\mathsf{V}_{X}
	\end{align}	
	%The matrices $(I-A\otimes A)$, $(I-(B+D)\otimes (B+D))$, $(I-D\otimes A)$, and $(I-A\otimes D)$ are full-rank with probability one. 
	By replacing $\mathsf{V}_{XZ}$ and $\mathsf{V}_{ZX}$ in terms of $\mathsf{V}_{Z}$ and $\mathsf{V}_{X}$, and then replacing $\mathsf{V}_{Z}$ in terms of $\mathsf{V}_{X}$ and $\mathsf{V}_{V}$, we can write:
	\begin{align}
	\mathsf{V}_X = R_1\mathsf{V}_{V} +R_2\mathsf{V}_{W},
	\end{align}	
	where each entry of $R_1$ and $R_2$ is a rational function $\frac{P}{Q}$, where $P$ and $Q$ are multivariate polynomials in entries of $A$, $B$ and $D$. As a result, each entry of $\Sigma_X$ can be written as a rational function, where both the nominator and the denominator are multivariate polynomials in entries of the system parameters $A$, $B$, $D$, $\Sigma_V$ and $\Sigma_W$. 
	Using Equ.~\ref{Eq:S6} and Equ.~\ref{Eq:S3} for $i=2$, we see that $\Sigma_{X_1}$ and $\Sigma_{X_2}$ are also rational functions of entries of the system parameters, and, as a result, $M_{12}$ and $M_{23}$ are.	
	Further, we can conclude that the $\det(M_{12})=\frac{P_1}{Q_1}$ and $\det(M_{23})=\frac{P_2}{Q_2}$, where $P_1$, $Q_1$, $P_2$ and $Q_2$ are multivariate polynomials in entries of the system parameters. 
	
	
	According to Lemma~\ref{lm:instance}, these multivarite polynomials are nonzero, because there exists an instance which results in a nonzero value for $\det(M_{12})$ and $\det(M_{23})$. Since the Lebesgue measure of roots of a nonzero multivariate polynomial is zero, we conclude that $\det(M_{12})$ and $\det(M_{23})$ are nonzero with probability one.
\end{proof}

\begin{lem}
	If $A$ is not full-rank, then $M_{23}$ is not full rank.
\end{lem}
\begin{proof}
	Using the Schur complement \cite[Schur]{} of $M_{23}$, we can write:
	\begin{align}
	\nonumber \mathrm{rank}(M_{23})=\mathrm{rank}(\Sigma_{X_1})+\mathrm{rank}(\Sigma_{X_1}-\Sigma_{X_2}\Sigma_{X_1}^{-1}\Sigma_{X}).
	\end{align}
	Using Equations \ref{Eq:S2} for $\tau=1$ and $2$, and Equ.~\ref{Eq:zx1}, we can write:
	\begin{align}
	\nonumber \Sigma_{X_1}-\Sigma_{X_2}\Sigma_{X_1}^{-1}\Sigma_{X}=A(\Sigma_{ZX}-\Sigma_{ZX_1}\Sigma_X^{-1}\Sigma_X).
	\end{align}
	Thus, if $A$ is not full-rank, $\Sigma_{X_1}-\Sigma_{X_2}\Sigma_{X_1}^{-1}\Sigma_{X}$, and, as a result, $M_{23}$ is also not full-rank. 
\end{proof}

Theorem~\ref{Th:M23} shows that if $A$ is full rank, we can use $M_{2,3}$ ro recover $K_1$ and $K_2$. However, depending on the values of $A$, $M_{2,3}$ might be very ill-conditioned. Thus, we use another equation.


\subsection{Second Equation} 

Combining Equ.~\ref{Eq:S6} and Equ.~\ref{Eq:S3} for $i=2$, we can write:
\begin{align}\label{Eq:Mat}
\begin{bmatrix}
\Sigma_{X_1} & \Sigma_{X_2}
\end{bmatrix}=
\begin{bmatrix}
K_1 & -K_2
\end{bmatrix}
M_{1,2}+
\begin{bmatrix}
-A\Sigma_W & 0
\end{bmatrix}
\end{align}
where
\begin{align}\label{Eq:Mat}
M_{1,2}=
\begin{bmatrix}
\Sigma_{X} & \Sigma_{X_{1}}\\
\Sigma_{X_{1}}^T  & \Sigma_{X} 
\end{bmatrix}.
\end{align}

%This matrix can be decomposed using the Schur complement:
%
%...
%
%and, therefore, we have:
%$$rank(M)=rank(\Sigma_{X})+rank(\Sigma_{X} - \Sigma_{X_1}\Sigma_{X}^{-1}\Sigma_{X_1}^T).$$
%Note that 
%$$\Sigma_{X_t|X_{t-1}}=\Sigma_{X} - \Sigma_{X_1}\Sigma_{X}^{-1}\Sigma_{X_1}^T.$$

What are the conditions such that we can recover the sparsity pattern of $D$?

\subsection{Algorithm}
\begin{itemize}
	\item Estimating the sparsity pattern of $D$. (what is the performance?)
	\item Relaxed LASSO: first find the SP using LASSO and then solve it using LS.
	\item Estimating $D$ and then $A$ and $B$. (Using cross-validation for estimating $A$?)
	\item Estimating the noise covariances.
	\item Use EM to further refine the estimation (?)
	\item Infer $z_t$ to be used for prediction.
\end{itemize}

%We can recover $K_1$ and $K_2$ as follows:
%$$
%\begin{bmatrix}
%K_1 & K_2
%\end{bmatrix}=
%\begin{bmatrix}
%\Sigma_{X_{t,t-3}} & \Sigma_{X_{t,t-2}}
%\end{bmatrix}
%M^{-1}.
%$$ 
%Since $CB+A$ is diagonal, using $K_1$, we can recover the off-diagonal elements of $D$. Then, using $K_2$, we can recover $A$, and, as a result, the entire $D$. Finally, $CB$ can be also recovered from $K_1$. 

%Assuming that B and D are diagonal, from identifiability, from equations in terms of B and DA+C, as well as DB and A. 

%Let $$Y_{U_1,U_2} = x_t-U_1x_{t-1}-U_2x_{t-2}.$$ We have: $$Y_{U_1,U_2} = ((K-U_1)C-U_2)x_{t-2}+((K-U_1)D+DB)z_{t-1}+(K-U_1)w_{t-1}+w_t+Dv_t$$ where $K=AD+C$.
%If we choose $(K-U_1)C-U_2 = 0$ and $(K-U_1)D+DB=0$, then $Y_{U_1,U_2}$ is pure noise and is independent of $x_{t-i}, i\geq 2$.
%For this, we should have: $U_1 = K+DBD^{-1}$ and $U_2 = -DBD^{-1}C$.


%We solve the following optimization problem:
%\begin{align}\label{Eq:Opt1}
% (K_1^*,K_2^*)=& argmin_{K_1, K_2} \|\Sigma_{X_{t,t-2}} - K_1\Sigma_{X_{t,t-1}} + K_2\Sigma_{X} \|_2^2  \\
%\nonumber & \mbox{s.t. } K_1 \mbox{ and } K_2 \mbox{ are sparse, with the same sparsity pattern.}
%\end{align}
%Then we let $CB+D+A=K_1^*$ and $AD = K_2^*$. 
%
%\textbf{How to set the sparsity patterns to be the same?}%
%...

%--------------------------------------------------------------------------------
%--------------------------------------------------------------------------------

%We can write:
%\begin{align}%\label{note1}
%\nonumber x_t = K_1x_{t-1}+K_2x_{t-2} +\mbox{noise}
%\end{align}
%where the noise term is not independent of the term $x_{t-1}$.
%Now, consider solving the following problem:
%\begin{align}%\label{note2}
%\nonumber [K_1^* \;\;\; K_2^*]=\mbox{argmin}_{K_1,K_2} \|x_t - (K_1x_{t-1}+K_2x_{t-2})\|_2^2.
%\end{align}
%The closed-form solution is as follows:
%\begin{align}
%\Sigma_{X_{t,t-2}} = K_1 \Sigma_{X_{t,t-1}} + K_2\Sigma_{X_{t,t}} \label{note3}\\ 
%\Sigma_{X_{t,t-1}} = K_1 \Sigma_{X_{t,t}}+ K_2 \Sigma_{X_{t,t-1}} ^T \label{note4}
%\end{align}
%
%The first equation is the same as our main equation. The second equation is wrong, where the correct from is: 
%\begin{align}
%\nonumber \Sigma_{X_{t,t-1}}  = K_1 \Sigma_{X_{t,t}}+ K_2 \Sigma_{X_{t,t-1}} ^T- A\Sigma_W %\label{note5}
%\end{align}
%
%However, the norm of the last term $(A\Sigma_W)$ is much smaller than other terms, and neglecting this term does not affect much the results.
%
%Equations \ref{note3} and \ref{note4} an be written as:
%\begin{align}
%[\Sigma_{X_{t,t-2}} \;\;\; \Sigma_{X_{t,t-1}}] = [K_1 \;\;\; K_2] M\label{note6}
%\end{align}
%where
%\begin{align}
%\nonumber M = 
%\begin{bmatrix}
%\Sigma_{X_{t,t-1}} &  \Sigma_{X_{t,t}}\\
%\Sigma_{X_{t,t}}  & \Sigma_{X_{t,t-1}}^T
%\end{bmatrix}.
%\end{align}
%
%With much smaller sample size, the results of solving Equ.~\ref{note6} are quite better than our current results. 

%--------------------------------------------------------------------------------
%--------------------------------------------------------------------------------


==> Sections/Other/Prelimiaries.tex <==
\section{Prelimiaries} 

\begin{lem}
	The following equality holds: \cite[petersen2008matrix]{keylist}
	\begin{equation}\label{Eq:kron}
	\mathsf{vec}(Q_1RQ_2)=(Q_2^T  \otimes Q_1)\mathsf{vec}(R)
	\end{equation}
	where $\mathsf{vec}$ is the vec-operator which stacks the columns of a matrix into a vector, $\otimes$ is the  Kronecker product, and $Q_1$, $Q_2$ and $R$ are square matrices with the same size. 
\end{lem}


\begin{lem}\cite[geiger2015causal]
	The set of zeros of any nonzero multivarite polynomial of degree $n$ has Lebesgue measure zero on $\mathbb{R}^n$.\label{lm:lebes}
\end{lem}

%\begin{lem}\cite[ouellette1981schur]{keylist}
%	Assume that $Q_i, 1\leq i \leq 4$, are square matrices with the same size, and assume that $Q_4$ is invertible. Using the Schur complement, we have:
%	\begin{align}
%	\nonumber &P=\left[\begin{matrix} Q_1 & Q_2 \\ Q_3 & Q_4 \end{matrix}\right] = \\
%	&\left[\begin{matrix} I & Q_2Q_4^{-1} \\ 0 & I \end{matrix}\right] \left[\begin{matrix} Q_1-Q_2Q_4^{-1}Q_3 & 0 \\ 0 & Q_4 \end{matrix}\right]
%	\left[ \begin{matrix} I & 0 \\ Q_4^{-1}Q_3 & I \end{matrix}\right].
%	\end{align}
%	We can also write:
%	\begin{align}\label{Eq:rank_schur}
%	\mathrm{rank}(P)=\mathrm{rank}(Q_4)+\mathrm{rank}(Q_1-Q_2Q_4^{-1}Q_3).
%	\end{align}
%\end{lem}




==> Sections/Other/Simulations_old.tex <==
\section{Simulations} 

\subsection{Condition Number}

Figure~\ref{fig:cond} show the condition number of matrices $M_{12}$ and $M_{23}$, with respect to changes in $A$, $B$ and $D$. In each case, we change one matrix and keep the other two matrices fixed. All settings are such that the system is stable. We average the results over 50 experiments. 

In simulations, we set $p=10$, $d=2$, $N=10^4$, $\Sigma_V=I$ and $\Sigma_W=I$. 
We have the following settings:

\begin{enumerate}
	\item $\|B\|_{Fro}=\|D\|_{Fro} = 0.15$ and $A=\alpha I$, where $\alpha=0.9^{1:50}$.
	\item $\|A\|_{Fro}=\|D\|_{Fro} = 0.11$ and $B=\beta I$, where $\beta=0.9^{1:50}$.
	\item $\|A\|_{Fro}=\|B\|_{Fro} = 0.20$, $\|D'\|_{Fro} = 2.2$ and $\|D\|_{Fro} = \gamma D'$, where $\gamma=0.9^{1:50}$.
\end{enumerate}


Figure~\ref{fig:cond} indicates that for most of the reasonable range of matrices $A$, $B$ and $D$, the matrix $M_{12}$ is well-conditioned; whereas $M_{23}$ is almost always ill-conditioned, unless if $A$ is the dominant parameter in the system.

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond12_A}
		\caption{Condition number of $M_{12}$ with respect to changes in $A$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond23_A}
		\caption{Condition number of $M_{23}$ with respect to changes in $A$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond12_B}
		\caption{Condition number of $M_{12}$ with respect to changes in $B$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond23_B}
		\caption{Condition number of $M_{23}$ with respect to changes in $B$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond12_D}
		\caption{Condition number of $M_{12}$ with respect to changes in $D$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/Cond23_D}
		\caption{Condition number of $M_{23}$ with respect to changes in $D$}
	\end{subfigure}
	\caption{Condition number of matrices $M_{12}$ and $M_{23}$, with respect to changes in the Frobenius norm of matrices $A$, $B$ and $D$.}\label{fig:cond}
\end{figure*}

\subsection{Comparisons}
We do three experiments. In each case, we set the Frobenius norm of two matrices to be the same and vary the Frobenius norm of the third one between $0.1$ to $10$ times of the one for the first two matrices.

We compare three methods. 1) Our proposed method, 2) EM, and 3) EM initialized with our method. 
We set $p=10$, $d=2$, $N=10^3$, $\Sigma_V=I$ and $\Sigma_W=I$. All settings are such that the system is stable. We initialize EM by $A=B=D=\frac{1}{2}I$ and $\Sigma_V=\Sigma_W=I$. We average the results over 20 experiments. 
Figures~\ref{fig:A}, \ref{fig:B} and \ref{fig:D} show the results.

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/A-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $A$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/A-error_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $A$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/A-error_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $A$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/A-error_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $A$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $A$.}\label{fig:A}
\end{figure*}


\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/B-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $B$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/B-error_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $B$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/B-error_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $B$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/B-error_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $B$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $B$.}\label{fig:B}
\end{figure*}

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/D-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $D$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/D-error_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $D$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/D-error_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $D$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=10/D-error_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $D$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $D$.}\label{fig:D}
\end{figure*}

%---------------------------------------------------------------------------------------------------

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $A$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-norm_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $A$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-norm_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $A$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-norm_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $A$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-norm_K1}
		\caption{Ratio of Frobenius norm of the error in $K_1$ with respect to changes in $A$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/A-norm_K2}
		\caption{Ratio of Frobenius norm of the error in $K_2$ with respect to changes in $A$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $A$ (20 nodes, $d=2$, average over 10 experiments).}\label{fig:A20}
\end{figure*}

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $B$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-norm_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $B$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-norm_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $B$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-norm_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $B$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-norm_K1}
		\caption{Ratio of Frobenius norm of the error in $K_1$ with respect to changes in $B$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/B-norm_K2}
		\caption{Ratio of Frobenius norm of the error in $K_2$ with respect to changes in $B$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $B$ (20 nodes, $d=2$, average over 10 experiments).}\label{fig:B20}
\end{figure*}

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-D}
		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $D$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-norm_A}
		\caption{Ratio of Frobenius norm of the error in $A$ with respect to changes in $D$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-norm_B}
		\caption{Ratio of Frobenius norm of the error in $B$ with respect to changes in $D$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-norm_D}
		\caption{Ratio of Frobenius norm of the error in $D$ with respect to changes in $D$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-norm_K1}
		\caption{Ratio of Frobenius norm of the error in $K_1$ with respect to changes in $D$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/p=20/D-norm_K2}
		\caption{Ratio of Frobenius norm of the error in $K_2$ with respect to changes in $D$}
	\end{subfigure}
	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $D$ (20 nodes, $d=2$, average over 10 experiments).}\label{fig:D20}
\end{figure*}

%---------------------------------------------------------------------------------------------------

%\begin{figure*}[hp]
%	\centering
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/SP_A}
%		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $A$}
%	\end{subfigure} \;\;\;\;\;
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/norm_A}
%		\caption{Ratio of Frobenius norm of the error with respect to changes in $A$}
%	\end{subfigure}\\
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/SP_B}
%		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $B$}
%	\end{subfigure}\;\;\;\;\;
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/norm_B}
%		\caption{Ratio of Frobenius norm of the error with respect to changes in $B$}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/SP_D}
%		\caption{Ratio of error in sign-sparsity pattern of $D$ with respect to changes in $D$}
%	\end{subfigure}\;\;\;\;\;
%	\begin{subfigure}[b]{0.45\linewidth}
%		\includegraphics[width=\linewidth]{Figures/norm_D}
%		\caption{Ratio of Frobenius norm of the error with respect to changes in $D$}
%	\end{subfigure}
%	\caption{Ratio of error in sign-sparsity pattern of $D$ and the ratio of Frobenius norm of the error with respect to changes in $A$, $B$ and $D$.}\label{fig:EM}
%\end{figure*}

\section{Results}

let $A$ sparse, $D=0$ and $B$ diagonal, $N=10^5$, $p=20$ and $s=2$. Results are averaged over 10 experiments. The pdf of $\tau$ is shown in Fig.~\ref{Fig:PDFtau}. Table~\ref{Table:Out_LASSO} shows the results.

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau1}
		\caption{$\mathbb{E}(\tau)=1$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau2}
		\caption{$\mathbb{E}(\tau)=2.4$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau3}
		\caption{$\mathbb{E}(\tau)=3.8$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau4}
		\caption{$\mathbb{E}(\tau)=5.3$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau5}
		\caption{$\mathbb{E}(\tau)=6.7$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau6}
		\caption{$\mathbb{E}(\tau)=8.1$}
	\end{subfigure}
	\caption{Histogram of $\tau$.}\label{Fig:PDFtau}
\end{figure*}

\begin{figure*}[hp]
	\centering
	\includegraphics[width=\linewidth]{Figures/PDFtau/Results}
	\caption{Ration of error in sign-sparsity pattern of $A$ versus the expected value of $\tau$.}\label{Fig:results}
\end{figure*}

%\begin{table*}[t]
%	\centering
%	\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c |}
%		\hline
%		$\mathbb{E}(\tau)$ & Our method & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10\\ \hline
%		\hline
%		1 & 0 & 0.16 & 0.07 & 0.11 & 0.23 & 0.35 & 0.54 & 0.68 & 0.80 & 0.93 & 1.04\\ \hline
%		2.4 & 0.09 & 0.41 & 0.29 & 0.21 & 0.19 & 0.24 & 0.30 & 0.38 & 0.46 & 0.53 & 0.62 \\ \hline
%		3.8 & 0.11 & 0.53 & 0.47 & 0.39 & 0.32 & 0.28 & 0.28 & 0.32 & 0.35 & 0.40 & 0.46 \\ \hline
%		5.3 & 0.11 & 0.59 & 0.56 & 0.52 & 0.46 & 0.39 & 0.34 & 0.33 & 0.35 & 0.39 & 0.43 \\ \hline
%		6.7 & 0.15 & 0.60 & 0.56 & 0.54 & 0.52 & 0.49 & 0.41 & 0.35 & 0.32 & 0.35 & 0.36 \\ \hline
%		8.1 & 0.14 & 0.67 & 0.64 & 0.63 & 0.64 & 0.63 & 0.58 & 0.51 & 0.43 & 0.38 & 0.36 \\ \hline
%		9.6 & 0.18 & 0.69 & 0.70 & 0.68 & 0.72 & 0.75 & 0.72 & 0.64 & 0.57 & 0.50 & 0.43 \\ \hline
%		11 & 0.23 & 0.64 & 0.64 & 0.64 & 0.67 & 0.71 & 0.73 & 0.70 & 0.62 & 0.56 & 0.48 \\ \hline
%	\end{tabular}
%	\caption{Our results versus LASSO for solving $\|\Sigma_{X_i} - A\Sigma_{X}\|+\lambda \|A\|_1$. Setting: $A$ sparse, $D=0$, $B$ diagonal, $N=10^5$, $p=20$ and $s=2$.}\label{Table:Out_LASSO}
%\end{table*}

==> Sections/Other/Structural.tex <==
\section{Structural Properties of the Model}

There are three important properties to look at in the state-space representation of time series: stability, controllability, and observability \cite{rangel2005modeling}. 
Let us define a new state vector to be $U_t = [z_t^T \; x_t^T]^T$. Then the model in Equ.~\ref{Eq:Mod1} can be written as:
\begin{align}\label{Eq:Mod1new}
U_{t+1}&=HU_{t}+N_{t+1}\\
x_t &= F U_t
\end{align}
where $F=[0 \; I]$, and $0$ and $I$ are $p\times p$ zero and identity matrices, respectively.

\subsection{Stability}  It must be ensured that the model does not cause the system to diverge to infinity. In order to maintain stability, we require that the spectral radius of the dynamics be less than or equal to 1. That is, we must have $\max(\lambda(H))\leq 1$, where $\lambda$ denotes the vector of eigenvalues for the matrix $H$.

\subsection{Controllability} Controllability is the requirement that the state vector $z_t$ can be controlled from any arbitrary initial state to any other arbitrary final state in finite time.
This would need to be accomplished by selecting $v_t$ to evolve in time in a particular way. Since we assume that the noise covariance for $v_t$ is nonsingular, the system is controllable if and only if $[I,H,H^2,\ldots,H^{2p-1}]$ is full rank. 

\subsection{Observability} Observability is the dual of controllability and is considered in terms of the observed variables $x_t$. We say that the system is observable if given zero noise, we can reconstruct the initial state vector from a full sequence of $x_t$.
This is achieved if and only if $[F^T,H^TF^T,(H^2)^TF^T,\ldots,(H^{2p-1})^TF^T]$ has full rank.

\subsection{Identifiability}
%Without loss of generality, we can set $z_t \leftarrow Cz_t$, $B \leftarrow CB$ and $v_t \leftarrow Cv_t$, and since $CAC^{-1}=A$, Equ.~\ref{Eq:Sys} can be written as:
%\begin{align}\label{Eq:Sys_C}
%\begin{cases}
%z_t = Az_{t-1} + Bx_{t-1} + v_t \\
%x_t = z_{t} + Dx_{t-1} + w_t.
%\end{cases}
%\end{align}


According to \cite{rangel2005modeling}, any coordinate transformation of hidden variables as $z'_t=Tz_t$, where $T$ is any nonsingular matrix, will generate observations that are identically distributed with those in Equ.~\ref{Eq:Sys}. As a result, it can be seen that
$$H'=
\begin{bmatrix}
TAT^{-1} & TB\\
CAT^{-1} & CB+D
\end{bmatrix}$$
generates the same distribution on observations as $H$ in Equ.~\ref{Eq:H}.

Since $A$ and $C$ are diagonal, $T$ can be only diagonal. Therefore, we have:
$$H'=
\begin{bmatrix}
A & TB\\
CAT^{-1} & CB+D
\end{bmatrix}.$$ 

If we set $C$ to be the identity matrix, then $T$ can be only identity. The modified model is:
\begin{align}\label{Eq:Mod}
\begin{cases}
z_t = Az_{t-1} + Bx_{t-1} + v_t \\
x_t = z_{t} + Dx_{t-1} + w_t
\end{cases}
\end{align}

Similar to Equ.~\ref{Eq:Mod1}, we can write:
\begin{align}\label{Eq:H2}
& \begin{bmatrix}
z_{t} \\
x_{t}
\end{bmatrix}=
H
\begin{bmatrix}
z_{t-1} \\
x_{t-1}
\end{bmatrix} 
+N_t
\end{align}
where 
\begin{align}\label{Eq:H}
H=\begin{bmatrix}
A & B\\
A & B+D
\end{bmatrix},
\end{align}
and $N_t =\begin{bmatrix}
v_{t} \\
w_t+v_{t}
\end{bmatrix}$
and therefore
$\Sigma_N =
\begin{bmatrix}
\Sigma_v & \Sigma_v\\
\Sigma_v & \Sigma_w+\Sigma_v^T
\end{bmatrix}.$\\


%\begin{align}\label{Eq:H2}
%H=\begin{bmatrix}
%A & B\\
%A & B+D
%\end{bmatrix}
%\end{align}
%In this case, the noise is 
%$N_t=\begin{bmatrix}
%v_{t} \\
%w_t+v_{t}
%\end{bmatrix}$, 
%and the noise covariance is
%$\Sigma_{N} =
%\begin{bmatrix}
%\Sigma_{v} & \Sigma_{v}\\
%\Sigma_{v} & \Sigma_w+\Sigma_{v}
%\end{bmatrix}$.



==> Sections/Other/Variations.tex <==
\newpage
\subsubsection{Other Variations} We have the following cases, based on the relative dimensions of $X$ and $Z$:

\textbf{Case $|Z|<<|X|:$} Now assume that $|Z|<<|X|$ and $A=\alpha I$. Using Equ.~\ref{Eq:S1}, we have:
$$\Sigma_{X_{t,t-2}} = (CB+D+\alpha I)\Sigma_{X_{t,t-1}} -\alpha D\Sigma_{X}.$$
This equation can be written as:
$$\Sigma_{X_{t,t-2}} = (L+S+\alpha I)\Sigma_{X_{t,t-1}} -\alpha S\Sigma_{X}$$
where $L$ and $S$ are low-rank and sparse matrices, respectively. Again, we can use 

\textbf{Case $B=0:$} If the state is evolved by itself, then $B=0$, and we have:
$$\Sigma_{X_{t,t-2}} = (D+CAC^{-1})\Sigma_{X_{t,t-1}} -CAC^{-1}D\Sigma_{X}.$$
Again, we can think about the following cases:
\begin{itemize}
	\item $|Z|=|X|$ and $A=\alpha I$: Special case of algorithm~\ref{Alg1}.
	\item $|Z|<<|X|$ and $A=\alpha I$: Write is as $\Sigma_{X_{t,t-2}} = (D+\alpha I)\Sigma_{X_{t,t-1}}-\alpha D\Sigma_{X}$.
\end{itemize}

\textbf{Case $D=0:$} If $X$ only depends on $Z$, then $D=0$, and we have:
$$\Sigma_{X_{t,t-2}} = (CB+CAC^{-1})\Sigma_{X_{t,t-1}}.$$
Again, we can think about the following cases:
\begin{itemize}
	\item $|Z|=|X|$ and $A=\alpha I$: Special case of algorithm~\ref{Alg1}.
	\item $|Z|<<|X|$ and $A=\alpha I$: Write is as $\Sigma_{X_{t,t-2}} = (CB+\alpha I)\Sigma_{X_{t,t-1}}$.
\end{itemize}


==> Sections/Other/time-var.tex <==
\section{Time-varying Model}

Assume that we have the following model:
\begin{align}\label{Eq:Sys}
\begin{cases}
z_t = Az_{t-1} + Bx_{t-1} + V_t \\
x_t = z_{t-\tau_t} + Dx_{t-1} + W_t
\end{cases}
\end{align}
where $\tau_t \in \{\mathbb{Z}\}^p$ is a random vector, with the constraint that for the $i$-th element we have $\tau_t^i \leq \tau_{t-1}^i+1$, meaning that once an observation depends on $z_{t_1}^i$, future observations can only depend on $z_{t_2}^i, t_2\geq t_1$.

For any fixed $\tau \geq 0$, we have:
\begin{align}
\Sigma_{X_{1}} &= (A+D)\Sigma_{X}-AD\Sigma_{X_{1}}^T+B\Sigma_{X_{\tau}}^T -A\Sigma_W \label{Eq:1}\\
\Sigma_{X_{i+1}} &= (A+D)\Sigma_{X_i}-AD\Sigma_{X_{i-1}}+B\Sigma_{X_{i-\tau}}, i\geq 1.\label{Eq:i}
\end{align}

For random $\tau$, we have to replace $\Sigma_{i-\tau}$ with $\mathbb{E}_{\tau}(\Sigma_{i-\tau})$. Therefore, we can write Equ.~\ref{Eq:i} as:
\begin{align}
\Sigma_{X_{i+1}} &= (A+D)\Sigma_{X_i}-AD\Sigma_{X_{i-1}}+B \sum_{j=0}^{\infty} {w_j\Sigma_{X_{i-j}}}, i\geq 1,
\end{align}
where $w_j=\Pr(\tau=j)$. 

I assume $D=0$, $B$ diagonal and $A$ to be sparse. Therefore, we have:
\begin{align}
B^{-1}\Sigma_{X_{i+1}} &= B^{-1}A\Sigma_{X_i} + \sum_{j=0}^{\infty} {w_j\Sigma_{X_{i-j}}}, i\geq 1.
\end{align}

Now, we can formulate a convex optimization problem in $L_1 =B^{-1}$, $L_2 = B^{-1}A$ and the vector of $w$. I did the simulations and the results are very good.


\section{Results}

let $A$ sparse, $D=0$ and $B$ diagonal, $N=10^5$, $p=20$ and $s=2$. Results are averaged over 10 experiments. The pdf of $\tau$ is shown in Fig.~\ref{Fig:PDFtau}. Table~\ref{Table:Out_LASSO} shows the results.

\begin{figure*}[hp]
	\centering
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau1}
		\caption{$\mathbb{E}(\tau)=1$}
	\end{subfigure} \;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau2}
		\caption{$\mathbb{E}(\tau)=2.4$}
	\end{subfigure}\\
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau3}
		\caption{$\mathbb{E}(\tau)=3.8$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau4}
		\caption{$\mathbb{E}(\tau)=5.3$}
	\end{subfigure}
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau5}
		\caption{$\mathbb{E}(\tau)=6.7$}
	\end{subfigure}\;\;\;\;\;
	\begin{subfigure}[b]{0.45\linewidth}
		\includegraphics[width=\linewidth]{Figures/PDFtau/PDFtau6}
		\caption{$\mathbb{E}(\tau)=8.1$}
	\end{subfigure}
	\caption{Histogram of $\tau$.}\label{Fig:PDFtau}
\end{figure*}

\begin{figure*}[hp]
	\centering
	\includegraphics[width=\linewidth]{Figures/PDFtau/Results}
	\caption{Ration of error in sign-sparsity pattern of $A$ versus the expected value of $\tau$.}\label{Fig:results}
\end{figure*}

%\begin{table*}[t]
%	\centering
%	\begin{tabular}{| c | c | c | c | c | c | c | c | c | c | c | c |}
%		\hline
%		$\mathbb{E}(\tau)$ & Our method & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10\\ \hline
%		\hline
%		1 & 0 & 0.16 & 0.07 & 0.11 & 0.23 & 0.35 & 0.54 & 0.68 & 0.80 & 0.93 & 1.04\\ \hline
%		2.4 & 0.09 & 0.41 & 0.29 & 0.21 & 0.19 & 0.24 & 0.30 & 0.38 & 0.46 & 0.53 & 0.62 \\ \hline
%		3.8 & 0.11 & 0.53 & 0.47 & 0.39 & 0.32 & 0.28 & 0.28 & 0.32 & 0.35 & 0.40 & 0.46 \\ \hline
%		5.3 & 0.11 & 0.59 & 0.56 & 0.52 & 0.46 & 0.39 & 0.34 & 0.33 & 0.35 & 0.39 & 0.43 \\ \hline
%		6.7 & 0.15 & 0.60 & 0.56 & 0.54 & 0.52 & 0.49 & 0.41 & 0.35 & 0.32 & 0.35 & 0.36 \\ \hline
%		8.1 & 0.14 & 0.67 & 0.64 & 0.63 & 0.64 & 0.63 & 0.58 & 0.51 & 0.43 & 0.38 & 0.36 \\ \hline
%		9.6 & 0.18 & 0.69 & 0.70 & 0.68 & 0.72 & 0.75 & 0.72 & 0.64 & 0.57 & 0.50 & 0.43 \\ \hline
%		11 & 0.23 & 0.64 & 0.64 & 0.64 & 0.67 & 0.71 & 0.73 & 0.70 & 0.62 & 0.56 & 0.48 \\ \hline
%	\end{tabular}
%	\caption{Our results versus LASSO for solving $\|\Sigma_{X_i} - A\Sigma_{X}\|+\lambda \|A\|_1$. Setting: $A$ sparse, $D=0$, $B$ diagonal, $N=10^5$, $p=20$ and $s=2$.}\label{Table:Out_LASSO}
%\end{table*}


